Hydrodynamic simulations of pulsar glitch recovery

Glitches are sudden jumps in the spin frequency of pulsars believed to originate in the superfluid interior of neutron stars. Superfluid flow in a model neutron star is simulated by solving the equations of motion of a two-component superfluid consisting of a viscous proton-electron plasma and an inviscid neutron condensate in a spherical Couette geometry. We examine the response of our model neutron star to glitches induced in three different ways: by instantaneous changes of the spin frequency of the inner and outer boundaries, and by instantaneous recoupling of the fluid components in the bulk. All simulations are performed with strong and weak mutual friction. It is found that the maximum size of a glitch that originates in the bulk decreases as the mutual friction strengthens. It is also found that mutual friction determines the fraction of the frequency jump which is later recovered, a quantity known as the 'healing parameter'. These behaviours may explain some of the diversity in observed glitch recoveries.

==> Untitled Folder/astromacros.tex <==
 \newcommand{\aj}{AJ}% Astronomical Journal 
 \newcommand{\araa}{ARA\&A}
 \newcommand{\apj}{ApJ}
 \newcommand{\apjl}{ApJ}
 \newcommand{\apjs}{ApJS}
 \newcommand{\ao}{Appl.~Opt.}
 \newcommand{\apss}{Ap\&SS}
 \newcommand{\aap}{A\&A}
 \newcommand{\aapr}{A\&A~Rev.}
 \newcommand{\aaps}{A\&AS}
 \newcommand{\azh}{AZh}
 \newcommand{\baas}{BAAS}
 \newcommand{\jrasc}{JRASC}
 \newcommand{\memras}{MmRAS}
 \newcommand{\mnras}{MNRAS}
 \newcommand{\pra}{Phys.~Rev.~A}
 \newcommand{\prb}{Phys.~Rev.~B}
 \newcommand{\prc}{Phys.~Rev.~C}
 \newcommand{\prd}{Phys.~Rev.~D}
 \newcommand{\pre}{Phys.~Rev.~E}
 \newcommand{\prl}{Phys.~Rev.~Lett.}
 \newcommand{\pasp}{PASP}
 \newcommand{\pasj}{PASJ}
 \newcommand{\qjras}{QJRAS}
 \newcommand{\skytel}{S\&T}
 \newcommand{\solphys}{Sol.~Phys.}
 \newcommand{\sovast}{Soviet~Ast.}
 \newcommand{\ssr}{Space~Sci.~Rev.}
 \newcommand{\zap}{ZAp}
 \newcommand{\nat}{Nature}
 \newcommand{\iaucirc}{IAU~Circ.}
 \newcommand{\aplett}{Astrophys.~Lett.}
 \newcommand{\apspr}{Astrophys.~Space~Phys.~Res.}
 \newcommand{\bain}{Bull.~Astron.~Inst.~Netherlands}
 \newcommand{\fcp}{Fund.~Cosmic~Phys.}
 \newcommand{\gca}{Geochim.~Cosmochim.~Acta}
 \newcommand{\grl}{Geophys.~Res.~Lett.}
 \newcommand{\jcp}{J.~Chem.~Phys.}
 \newcommand{\jgr}{J.~Geophys.~Res.}
 \newcommand{\jqsrt}{J.~Quant.~Spec.~Radiat.~Transf.}
 \newcommand{\memsai}{Mem.~Soc.~Astron.~Italiana}
 \newcommand{\nphysa}{Nucl.~Phys.~A}
 \newcommand{\physrep}{Phys.~Rep.}
 \newcommand{\physscr}{Phys.~Scr}
 \newcommand{\planss}{Planet.~Space~Sci.}
 \newcommand{\procspie}{Proc.~SPIE}
 \newcommand{\nar}{New Astronomy Reviews}
 \newcommand{\astroussr}{Astronomical Circular U.S.S.R.}
 \newcommand{\royalsoc}{The Royal Society}

